Counting with Focus for Free

This paper aims to count arbitrary objects in images. The leading counting approaches start from point annotations per object from which they construct density maps. Then, their training objective transforms input images to density maps through deep convolutional networks. We posit that the point annotations serve more supervision purposes than just constructing density maps. We introduce ways to repurpose the points for free. First, we propose supervised focus from segmentation, where points are converted into binary maps. The binary maps are combined with a network branch and accompanying loss function to focus on areas of interest. Second, we propose supervised focus from global density, where the ratio of point annotations to image pixels is used in another branch to regularize the overall density estimation. To assist both the density estimation and the focus from segmentation, we also introduce an improved kernel size estimator for the point annotations. Experiments on six datasets show that all our contributions reduce the counting error, regardless of the base network, resulting in state-of-the-art accuracy using only a single network. Finally, we are the first to count on WIDER FACE, allowing us to show the benefits of our approach in handling varying object scales and crowding levels. Code is available at https://github.com/shizenglin/Counting-with-Focus-for-Free

==> wider-face.tex <==
%===============================
\section{Counting on WIDER-FACE}
%===============================
WIDER FACE dataset~\cite{yang2016wider} is a recently released large-scale face detection benchmark. In this paper, we reuse this data for face counting as a complementary crowd dataset. Compared to the existing crowd dataset like ShanghaiTech~\cite{zhang2016single}, WIDER FACE dataset is more challenging due to large variations in scale, occlusion, pose, and background clutter. Moreover, it contains more images, in a total of $32,203$ images. $40\%/10\%/50\%$ of the data is randomly selected for training, validation, and testing, respectively. Groundtruth of testing dataset is unavailable, so we use the training dataset for training, and validation dataset for testing. Each face in images of this dataset is annotated by a bounding box, instead of a point annotation, so we can easily know the size of face according to the bounding box, which allows us evaluate various methods from multiple conditions such as scale, congestion and event. Moreover, we can evaluate our proposed new density kernel with the bounding box.  

\textbf{Baseline.} For this new counting dataset, we choose these three methods which are proposed by Zhang \etal \cite{zhang2016single}, Li \etal \cite{Li_2018_CVPR} an Cao \etal \cite{Cao_2018_ECCV} because they achieved the state-of-the-art performance on ShanghaiTech dataset, as the baseline methods. We also compare our proposed method with these three methods. To further demonstrate that the proposed method is complementary to the existing methods, we combine the proposed focus with these three baseline methods.  

\textbf{Overall.} In this dataset, we use MAE as the metric to evaluate various methods. However, ,we propose a new metric named Normalized Mean Average Error (NMAE). To make each image equally treated avoiding the effect of count, we normalize the MAE of each image by their count. The results in terms of MAE and NMAE are shown in Table~\ref{tab_overall}.

\begin{table}[t]
\centering
\caption{\textbf{Overall performance} on WIDER-FACE.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
 & \multicolumn{2}{c}{Zhang \etal \cite{zhang2016single}} & \multicolumn{2}{c}{Li \etal \cite{Li_2018_CVPR}} &
 \multicolumn{2}{c}{Cao \etal \cite{Cao_2018_ECCV}} & \multicolumn{2}{c}{\textit{This paper}}\\
 \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
 & MAE & NMAE & MAE & NMAE & MAE & NMAE & MAE & NMAE\\
\midrule
Base Network & 7.1 & 1.1 & 8.5 & 1.1 & 4.3 & 0.53 & 4.7 & 0.91\\
\midrule
+Focus & \textbf{6.1} & \textbf{1.0} & \textbf{8.3} & \textbf{0.67} & \textbf{-} & \textbf{-} &\textbf{3.2} & \textbf{0.40}\\
\bottomrule
\end{tabular}}
\label{tab_overall}
\end{table}



\begin{table}[t]
\centering
\caption{\textbf{Scale performance} on WIDER-FACE.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lccccccccccc}
\toprule
 & & \multicolumn{2}{c}{Zhang \etal \cite{zhang2016single}} & \multicolumn{2}{c}{Li \etal \cite{Li_2018_CVPR}} &
 \multicolumn{2}{c}{Cao \etal \cite{Cao_2018_ECCV}} & \multicolumn{2}{c}{\textit{This paper}}\\
 \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
 & & MAE & NMAE & MAE & NMAE & MAE & NMAE & MAE & NMAE\\
\midrule
\multirow{3}{*}{Base Network}&Small& - & - & - & - & - & - & - & -\\
                             &Medium& - & - & - & - & - & - & - & -\\
                             &Large& - & - & - & - & - & - & - & -\\
\midrule
\multirow{3}{*}{+Focus}&Small& - & - & - & - & - & - & - & -\\
                             &Medium& - & - & - & - & - & - & - & -\\
                             &Large& - & - & - & - & - & - & - & -\\
\bottomrule
\end{tabular}}
\label{tab_scale}
\end{table}

  

\begin{table}[t]
\centering
\caption{\textbf{Congestion performance} on WIDER-FACE.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lccccccccccc}
\toprule
 & & \multicolumn{2}{c}{Zhang \etal \cite{zhang2016single}} & \multicolumn{2}{c}{Li \etal \cite{Li_2018_CVPR}} &
 \multicolumn{2}{c}{Cao \etal \cite{Cao_2018_ECCV}} & \multicolumn{2}{c}{\textit{This paper}}\\
 \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
 & & MAE & NMAE & MAE & NMAE & MAE & NMAE & MAE & NMAE\\
\midrule
\multirow{3}{*}{Base Network}&Sparse& - & - & - & - & - & - & - & -\\
                             &Medium& - & - & - & - & - & - & - & -\\
                             &Dense& - & - & - & - & - & - & - & -\\
\midrule
\multirow{3}{*}{+Focus}&Sparse& - & - & - & - & - & - & - & -\\
                             &Medium& - & - & - & - & - & - & - & -\\
                             &Dense& - & - & - & - & - & - & - & -\\
\bottomrule
\end{tabular}}
\label{tab_congestion}
\end{table}

\textbf{Event} Different events are typically associated with different scenes. WIDER FACE contains 60 event categories covering a large number of scenes in the real word. To evaluate the influence of event to face counting, we compare various methods in three portions of events: easy events (41-60 classes), medium (21-40 classes) and hard (1-20 classes), which is grouped by the work in ~\cite{yang2016wider}. The results are shown in Table~]\ref{tab_event}. The results for three parts are shown in Table~\ref{tab_congestion}.

\begin{table}[t]
\centering
\caption{\textbf{Event performance} on WIDER-FACE.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lccccccccccc}
\toprule
 & & \multicolumn{2}{c}{Zhang \etal \cite{zhang2016single}} & \multicolumn{2}{c}{Li \etal \cite{Li_2018_CVPR}} &
 \multicolumn{2}{c}{Cao \etal \cite{Cao_2018_ECCV}} & \multicolumn{2}{c}{\textit{This paper}}\\
 \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10}
 & & MAE & NMAE & MAE & NMAE & MAE & NMAE & MAE & NMAE\\
\midrule
\multirow{3}{*}{Base Network}&Easy& - & - & - & - & - & - & - & -\\
                             &Medium& - & - & - & - & - & - & - & -\\
                             &Hard& - & - & - & - & - & - & - & -\\
\midrule
\multirow{3}{*}{+Focus}&Easy& - & - & - & - & - & - & - & -\\
                             &Medium& - & - & - & - & - & - & - & -\\
                             &Hard& - & - & - & - & - & - & - & -\\
\bottomrule
\end{tabular}}
\label{tab_event}
\end{table}

\textbf{Kernel Comparison}

\begin{table}[!t]
\small
\centering
\caption{\textbf{Kernel comparison} on WIDER-FACE.}
\begin{tabular}{@{}ccccccc@{}}
\toprule
 & \multicolumn{3}{c}{\textbf{Metrics}}   \\
 \cmidrule(lr){2-4}
 & MAE & NMAE & MAE($\sigma$) \\
\hline
GAK~\cite{zhang2016single} &- & - & -  \\
LIK(\textit{this paper}) & - & - & - \\
Grounttruth & - & - & - \\
\bottomrule
\end{tabular}
\label{tab_kernel}
\end{table}
